Conversational Recommender System and Large Language Model Are Made for Each Other in E-commerce Pre-sales Dialogue

E-commerce pre-sales dialogue aims to understand and elicit user needs and preferences for the items they are seeking so as to provide appropriate recommendations. Conversational recommender systems (CRSs) learn user representation and provide accurate recommendations based on dialogue context, but rely on external knowledge. Large language models (LLMs) generate responses that mimic pre-sales dialogues after fine-tuning, but lack domain-specific knowledge for accurate recommendations. Intuitively, the strengths of LLM and CRS in E-commerce pre-sales dialogues are complementary, yet no previous work has explored this. This paper investigates the effectiveness of combining LLM and CRS in E-commerce pre-sales dialogues, proposing two collaboration methods: CRS assisting LLM and LLM assisting CRS. We conduct extensive experiments on a real-world dataset of Ecommerce pre-sales dialogues. We analyze the impact of two collaborative approaches with two CRSs and two LLMs on four tasks of Ecommerce pre-sales dialogue. We find that collaborations between CRS and LLM can be very effective in some cases.

==> sections/5-Results-backup.tex <==
\section{Results and Analysis}
\label{sec:results}
% We present the experimental results and analysis by tasks.
% For each task, we first present the performance of the baseline and collaborative approaches on the task, and then analyze the effects of the collaborative approach.
\subsection{Overall performance}
\label{sec:resutls_rq1}
We start with RQ1. 
Specifically, we first analyze the performance of LLM and CRS separately.
Then we analyze the performance of the two combined.

\header{Overall performance of \acp{CRS}}
% Performance of \acp{LLM} on the pre-sales dialogue understanding task.
% From Table~\ref{tab:experiment_task1}, we observe that:
% (1) xxxxxxx
% (2) xxxxxxxxxx
% (3) xxxxxxxxxx.
According to the results in Tables~\ref{tab:experiment_task1} to ~\ref{tab:experiment_task4}, when there is no collaboration, we observe that CRS methods have good performance on user needs elicitation (task 3) and user needs-based recommendation (task 2). Specifically, on task 2, UniMIND (BART) achieves the best results on the shoes category, the cell phone category, and all categories. On Task 3, UniMIND(CPT) and UniMIND(BART) obtain the best as well as the second best results on all categories.
LLM is capable of achieving a certain performance after task fine-tuning. However, CRS is more advantageous on classification tasks or ranking tasks that require analysis of intrinsic connections.

\header{Overall performance of \acp{LLM}}
Based on the results in Tables~\ref{tab:experiment_task1} to ~\ref{tab:experiment_task4}, we see that the LLM approach has good performance on pre-sales dialogue understanding (task 1) and pre-sales dialogue generation (task 4) when there is no collaboration. Specifically, the fine-tuned ChatGLM-6B achieves the best results on all metrics for all categories.
We attribute this to the fact that tasks 1 and 4 require language capability, and the larger model has superb language capability.


\header{Overall performance of combining of \acp{LLM} and \acp{CRS}}
From the results in Tables~\ref{tab:experiment_task1} to ~\ref{tab:experiment_task4}, we observe that the combined LLM and CRS approach achieves good performance on all tasks.
Specifically, on task 1, BCRS-CLLM achieves the best results on most of the metrics.
On Task 2, CLLM-BCRS achieved the best results on most of the metrics.
On Task 3, CLLM-CCRS achieved the best results on most of the metrics.
On task 4, BCRS-ALLM achieved the best results on both automatic and manual evaluations.

Based on the above results, we find that the large model has better performance on the language-related tasks 1 and 4, but the performance is limited when modeling relational sorting classification is required. And CRS has better performance on tasks 2 and 3, but limited performance on tasks 1 and 4.
When the two are combined, they perform well on all tasks.
Therefore, we conclude that LLM and CRS are complementary in the pre-sales dialogue scenarios.

\subsection{Analysis of combinations of \acp{LLM} and \acp{CRS}}
\label{sec:resutls_rq2}
For RQ2 we investigate the impact of (1) the combination approach and (2) the different base models on the performance.
We analyze both from the task and category perspectives.

\header{Impact of collaborative approach}
We investigate the effects of the two combinations on the four tasks.
Based on the results in Tables 1 through 4, we find that:
(1) The choice of combining methods needs to consider the features of the task and the categories involved. If model A has a better performance on that task, B provides information to A is likely to improve the performance. Conversely, there may not be a large boost.
(2) We do not observe a more consistent phenomenon on different categories.
For example, for task 1, LLM assists CRS better than CRS assists LLM in the beauty category, while the exact opposite is observed in the Shoes category.
We believe this is due to the large differences in categories, which also reflects the complexity of real scenarios and future research points worth exploring.


\header{Impact of base model}
We investigate the effects of 2 types of CRS combined with 2 types of LLM on 4 tasks.
CPT can be directly applied to natural language understanding and natural language generation tasks, while BART is only applicable to natural language generation by default.
Chinese-alpaca is an extension of llama with Chinese language capability.
While ChatGLM uses training techniques similar to ChatGPT e.g., RLHF.
According to the results in Tables 1 to 4, when model A is fixed and model B is different, we find that:
(1)
